Large Language Models Penetration in Scholarly Writing and Peer Review

While the widespread use of Large Language Models (LLMs) brings convenience, it also raises concerns about the credibility of academic research and scholarly processes. To better understand these dynamics, we evaluate the penetration of LLMs across academic workflows from multiple perspectives and dimensions, providing compelling evidence of their growing influence. We propose a framework with two components: \texttt{ScholarLens}, a curated dataset of human- and LLM-generated content across scholarly writing and peer review for multi-perspective evaluation, and \texttt{LLMetrica}, a tool for assessing LLM penetration using rule-based metrics and model-based detectors for multi-dimensional evaluation. Our experiments demonstrate the effectiveness of \texttt{LLMetrica}, revealing the increasing role of LLMs in scholarly processes. These findings emphasize the need for transparency, accountability, and ethical practices in LLM usage to maintain academic credibility.

==> section/02-rw.tex <==


\section{Related works}




In recent years, discussions in the scientific community have focused on improving the peer review process~\cite{gurevych_et_al:DagRep.14.1.130, kuznetsov2024natural} to address issues like misalignment between reviewers and paper topics, as well as social~\cite{huber2022nobel, tomkins2017reviewer, manzoor2021uncovering} and cognitive biases~\cite{lee2015commensuration, stelmakh2021prior}. Proposed solutions include enhancing structural incentives for reviewers~\cite{rogers-augenstein-2020-improve}, using natural language processing for intelligent support~\cite{kuznetsov-etal-2022-revise, zyska-etal-2023-care, dycke-etal-2023-nlpeer, guo-etal-2023-automatic, kumar-etal-2023-reviewers}, and other policy recommendations~\cite{dycke-etal-2022-yes}. Additionally, some studies focus on the collection and analysis of review data~\cite{kennard-etal-2022-disapere, staudinger-etal-2024-analysis, darcy-etal-2024-aries}.\footnote{\href{https://arr-data.aclweb.org/}{ACL Rolling Review Data Collection (ARR-DC)}.} 
\textbf{However, these efforts largely center on human reviewers—what if, instead, the reviewers are AI?}


The recurrent use of specific syntactic templates in LLM-generated text largely reflects patterns from the training data~\cite{shaib-etal-2024-detection}, highlighting the model's memorization capacity~\cite{karamolegkou-etal-2023-copyright, zeng-etal-2024-exploring, zhu-etal-2024-beyond}.






AgentReview~\cite{jin2024agentreview}

BUST: Benchmark for the evaluation of detectors of LLM-Generated Text~\cite{cornelius-etal-2024-bust}


\subsection{Large Language Models Penetration}


\lz{\cite{wei2024understanding}: this paper performs the first analysis of the impact that AIGC has had on the social media ecosystem, through the lens of Pixiv.}

With the rapid development of large language models (LLMs), the penetration of LLM technology into various fields has deepened,and especially academia, such as science journal writing~\cite{jiang2024llm}, Academic information seeking~\cite{wang2024solution} by using a SOAY tool to enhances LLMs' academic paper retrieval, and peer review generation tasks~\cite{su-etal-2023-reviewriter},
which provides a tool for writing peer reviews in German.
Simultaneously, some related studies have proposed methods utilizing large language models (LLMs) to facilitate the work of paper reviewers.
~\cite{weber2024other} provide a fine-tuned model used to automate peer reviews which is named RoboReviewe,
and ~\cite{gao2024reviewer2optimizingreviewgeneration} purpose propose an efficient two-stage review generation framework for helping reviewer to find the deficiency of the sketched review.
Meanwhile, ~\cite{santu2024promptingllmscomposemetareview} Introduced a method to compose meta-review drafts from peer-review narratives.

Although the use of LLM-generated review/meta-review has facilitated the paper review process,
the widespread application of these technologies raises concerns about the level of engagement and
effort put in by reviewers. 
~\cite{jin-etal-2024-agentreview} reported that 15.8\% of ICLR 2024 reviews were AI-assisted, with AI-assisted reviews consistently assigning higher scores than their human counterparts and AI-assisted reviews contributed to a 4.9 percentage point increase in acceptance rates for borderline submissions.
~\cite{du-etal-2024-llms} collaborated with 40 experts in LLM-related reviewing to conduct a fine-grained evaluation of reviews generated by LLMs.
Moreover, ~\cite{zhou-etal-2024-llm} shows that LLM generate review prefers excessively positive word than human.
both of them reveal a signal of the importance to investigate the involvement of AI in the this process.In this work, we make a distinction from previous studies by focusing on the participation rate of AI-generated text in the paper review process.

LLMs have developed a strong capability in text generation tasks. Specifically in the academic domain, \cite{birhane2023science} have highlighted the convenience of LLMs in peer review and abstract writing. During the peer review process, some reviewers utilize LLMs for summary tasks to aid in reading, and even instruct LLMs to generate review sketches\cite{zou2024chatgpt}. Additionally, some meta-reviewers will employ LLMs to summarize reviewers' suggestions for creating meta-reviews\cite{santu2024prompting}. However, the summary results produced by LLMs may not fully capture the research information of a paper. Reviewers who overly rely on these summary results may compromise the objectivity and authenticity of the review process.

On the other hand, in abstract writing tasks, LLMs are often used for polishing and text completion\cite{khalifa2024using}, such as generating the Background for the abstract. This, however, poses the risk of making published outputs more uniform, potentially reducing the distinctive voice and style of human-authored works. In above, We believe that studying the penetration of LLMs from these two aspects can effectively reflect the extent of LLM penetration in academia.
% \lz{Summarize current research on LLM penetration across multiple domains, particularly highlighting advancements and impacts within the academic domain.}

% \lz{Perhaps we can summarize an analytical perspective of the existing work and compare it}



\subsection{Evaluation Metric}

% \lz{@Li Zhou: including Detection Model, Linguistic Feature metric, and so on}

% candidate:
% automatic metric: BLEU, ROUGE, ……
% Linguistic Features: ……


==> table/direct_linguist_feature.tex <==
\begin{table}[ht]
% \setlength{\tabcolsep}{2.5pt} % Adjust column padding to fit content better
\centering
\footnotesize 
\begin{tabular}{@{}l@{}}
\toprule
\textbf{Structural Features} \\ \midrule
Average Word length \\
Average Sentence length \\
Average Words per sentence \\
Average Number of Words \\
Average Number of Sentences \\

\toprule
\textbf{Lexical Features} \\ \midrule
Percent of unique words \\
Percent of long words \\
Percent of stopwords \\
Vocabulary Richness \\

\toprule
\textbf{Linguistic Quality Features} \\ \midrule
Syntactic Diversity \\
Readability \\
Fluency \\

\bottomrule
\end{tabular}
\caption{Direct Linguistic Features}
\label{tab:Direct_Linguistic_Features}
\end{table}


==> table/direct_linguist_feature_description.tex <==
\begin{table*}[ht]
\centering
\footnotesize 
\begin{tabular}{@{}l|p{0.4\textwidth}|p{0.4\textwidth}@{}}
\toprule
\textbf{Structural Features}         & \textbf{Description} & \textbf{Computing Method} \\ \midrule
\textbf{Average Word Length}          & Measures the average number of characters in each word in the text. &  \\ 
\textbf{Average Sentence Length}       & Measures the average number of words in each sentence in the text. &  \\ 
\textbf{Average Number of Words} & Counts the average total words in the text. &  \\ 
\textbf{Average Number of Sentences}     & Counts the average total sentences in the text. &  \\ \midrule




\textbf{Lexical Features}          \\ \midrule
\textbf{Percent of Long Words}   & Measures the percentage of “long words” in the text. We define long words as words with more than 6 letters. & $\text{Percent of Long Words} = \left(\frac{\text{Long Words}}{\text{Total Words}}\right) \times 100\%$ \\ 
\textbf{Percent of Stopwords}   & Measures the percentage of common words in the text, like "the," "and," and "is." A high percentage means the text has more filler words. & $\text{Percent of Stopwords} = \left(\frac{\text{Stopwords}}{\text{Total Words}}\right) \times 100\%$ \\ 
\textbf{Vocabulary Richness}   & Measures how many unique words are used compared to the total number of words. "Unique words" are the different words that appear in a text, without counting repeats. 

For example, in “apple orange apple,” there are 3 words, but only 2 unique words: "apple" and "orange."

A higher ratio means the text has more varied vocabulary. & $\text{Vocabulary Richness} = \frac{\text{Unique Words}}{\text{Total Words}}$  \\ \midrule




\textbf{Linguistic Quality Features}         \\ \midrule
\textbf{Syntactic Diversity} & Syntactic diversity assesses structural complexity by examining clause patterns. &  \\ 
\textbf{Readability} & Readability indices measure how easily a reader can understand a written text. We use the following metrics to measure readability:

-Flesch-Kincaid Scores: Measures how easy the text is to read, based on sentence length and word syllables.

-Flesch Scores: Rates how easy or hard the text is to read for different age levels.

-Gunning Fog Scores: Shows the education level needed to understand the text.

-Coleman-Liau Scores: Uses word and sentence length to tell what grade level can read the text.

-Dale-Chall Scores: Rates readability based on the use of familiar or common words.

-ARI Scores: Estimates readability using the number of characters and words.

-Linsear Write Scores: Measures readability by looking at sentence structure and word difficulty.
&

We use the \text{textstat} library directly to calculate these seven metrics. The specific calculation formulas are as follows:

\text{Flesch-Kincaid Grade Level} = 

$0.39 \times \frac{\text{Total Words}}{\text{Total Sentences}} + 11.8 \times \frac{\text{Total Syllables}}{\text{Total Words}} - 15.59 $
\medskip

\text{Flesch Reading Ease} = 

$206.835 - 1.015 \times \frac{\text{Total Words}}{\text{Total Sentences}} - 84.6 \times \frac{\text{Total Syllables}}{\text{Total Words}}$ 
\medskip

\text{Gunning Fog Index} = 

$0.4 \times \left( \frac{\text{Total Words}}{\text{Total Sentences}} + 100 \times \frac{\text{Complex Words}}{\text{Total Words}} \right)$ 
\medskip

\text{Coleman-Liau Index} = 

$0.0588 \times \text{Average Number of Letters per 100 Words} - 0.296 \times \text{Total Sentences} - 15.8$ 
\medskip

\text{Dale-Chall Readability Score} = 

$0.1579 \times \frac{\text{Difficult Words}}{\text{Total Words}} + 0.0496 \times \frac{\text{Total Words}}{\text{Total Sentences}} + 3.6365 $
\medskip

\text{Automated Readability Index (ARI)} =

$4.71 \times \frac{\text{Total Characters}}{\text{Total Words}} + 0.5 \times \frac{\text{Total Words}}{\text{Total Sentences}} - 21.43$ 
\medskip

\text{Linsear Write Formula} = 
$\frac{\left( \text{Easy Words} + 3 \times \text{Difficult Words} \right)}{\text{Total Sentences}}$




\\ 
\textbf{Fluency} & Fluency is the quality of a text based on how well it is written and whether it is grammatically correct. & this may be abandoned \\ 




\bottomrule
\end{tabular}
\caption{Direct Linguistic Features with brief descriptions}
\label{tab:Direct_Linguistic_Features_description}
\end{table*}


==> table/indirect_feature.tex <==
\begin{table}[ht]
% \setlength{\tabcolsep}{2.5pt} % Adjust column padding to fit content better
\centering
\footnotesize 
\begin{tabular}{@{}l@{}}

\toprule
\textbf{writers' attitude} \\ \midrule
Emotions \\
Persuasiveness \\
Convincingness\\


\toprule
\textbf{relatedness} \\ \midrule



\bottomrule
\end{tabular}
\caption{Indirect Features}
\label{tab:Indirect_Features}
\end{table}


==> table/indirect_features_description.tex <==
\begin{table*}[ht]
\centering
\footnotesize 
\begin{tabular}{@{}l|p{0.4\textwidth}|p{0.4\textwidth}@{}}
\toprule
\textbf{Relatedness}         & \textbf{Description} & \textbf{Computing Method} \\ \midrule
\textbf{bert score}      
 &BERT score is a metric that evaluates the alignment between two texts by comparing their contextual embeddings. It compares words in the candidate text with words in the reference text one by one, accumulating word vector similarities to get an overall similarity score. Precision, Recall, and F1 scores are calculated separately. We compute the BERT score between the meta-review and the three reviews, then compute the average and variance to measure their similarity.  &The BERT score between two texts is typically calculated using the cosine similarity of their contextual embeddings. Given a reference text R(here is review) and a candidate text C(here is meta-review), BERT score evaluates Precision, Recall, and F1 metrics as follows:  
 
\text{Precision (P)}

$P = \frac{1}{|C|} \sum_{c \in C} \max_{r \in R} \text{cos\_sim}(c, r)$ 
\medskip

\text{Recall (R)}

$R = \frac{1}{|R|} \sum_{r \in R} \max_{c \in C} \text{cos\_sim}(r, c)$ 
\medskip

\text{F1 Score}

$F1 = \frac{2 \cdot P \cdot R}{P + R}$ 
 \\ 
\textbf{sentence bert}       & Sentence-BERTScore is a metric that evaluates the alignment between two texts by comparing their contextual embeddings, optimized for sentence-level similarity. It encodes each sentence or short text into a single vector for the whole sentence, then calculates the similarity between two sentence vectors (with cosine similarity) to measure how similar the sentences are. We compute the Sentence-BERTScore between the meta-review and each of the three reviews, then calculate the average and variance to measure their overall similarity. &  
$\mathbf{E}_{\text{meta-review}}$ represents the sentence embedding of the meta-review.
$\mathbf{E}_{\text{review}}$ represents the sentence embedding of a single review.

\text{Similarity} = 
$\frac{\mathbf{E}_{\text{meta-review}} \cdot \mathbf{E}_{\text{review}}}{\|\mathbf{E}_{\text{meta-review}}\| \|\mathbf{E}_{\text{review}}\|}$

\\ 
\midrule

\textbf{Writers' attitude}          & &  \\ \midrule
\textbf{Emotions}   &Measure the distribution of emotions in the text. There are various types of emotions, such as disappointment, sadness, annoyance, joy, anger, caring, optimism, curiosity, gratitude, and more. These emotions cover a range from positive to negative, helping us to understand the emotional tone and intent of the writing. & We use $SamLowe/roberta-base-go\_emotions$,a model trained on the Go-Emotions dataset to classify over 28 emotions. \\

\textbf{Persuasiveness}   &Binary classification (Non-persuasive, Persuasive)
 &To finish the task, we use the $paragon-analytics/roberta\_persuade model$, a binary classifier, to finish this task.\\ 
\textbf{Convincingness}   &Binary classification (Non-Convincingness, Convincingness) &To finish the task, we use $jakub014/bert-base-uncased-IBM-argQ-30k-finetuned-convincingness-IBM$, a model trained on the assumption that convincingness is linked to
high quality arguments which are typically clear, relevant, and with high impact.\\ \midrule


\bottomrule
\end{tabular}
\caption{Indirect Features with brief descriptions}
\label{tab:Indirect_Linguistic_Features_description}
\end{table*}


==> table/linguistic_features.tex <==
\begin{table}[ht]

% \setlength{\tabcolsep}{2.5pt} % Adjust column padding to fit content better
\centering
\footnotesize 
\begin{tabular}{@{}l|r@{\hskip 2mm}r@{\hskip 2mm}r@{\hskip 2mm}r@{}}
\toprule
\textbf{Feature}         & \textbf{Human}         & \textbf{AI}           \\ \midrule
\textbf{Avg. Word Count}          & 106.96±84.94 & 114.03±69.60 \\
\textbf{Avg. Sent. Count}       & 5.33±4.19   & 6.78±3.83  \\
\textbf{Senti. Polar. Score} & 0.13±0.13    & 0.12±0.09    \\
\textbf{Gram. Errors} & 18.22±20.60   & 8.28±11.42    \\
\textbf{Synt. Diversity} & 1.12±0.77   & 0.65±0.37    \\
\textbf{Voca. Richness}   & 0.77±0.11     & 0.81±0.09    \\
\textbf{Read. Score}     & 18.49±4.05    & 22.33±2.20    \\
\bottomrule
\end{tabular}
\caption{Feature differences between meta-review. The value in the corresponding cell indicates the mean ± standard deviation.}
\label{tab:feature_comparison}
\end{table}

==> table/polishing_prompt.tex <==
% \begin{table}[ht]
% \centering
% \footnotesize
% \begin{tabular}{@{}p{0.8\textwidth}@{}}
% \toprule
% \textbf{Prompts} \\ \midrule
% Can you help me revise the abstract? Please response directly with the revised abstract: {abstract} \\
% please revise the abstract, and response directly with the revised abstract: {abstract} \\
% Can you check if the flow of the abstract makes sense? Please response directly with the revised abstract: {abstract} \\
% Please revise the abstract to make it more logical, response it directly with the revised abstract: {abstract} \\
% Please revise the abstract to make it more formal and academic, response it directly with the revised abstract: {abstract}\\
% \bottomrule
% \end{tabular}
% \caption{Polishing Prompts}
% \label{tab:polishing_prompts}
% \end{table}

==> table/training_args.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    \begin{tabular}{@{}l|r@{}}
        \toprule
        \textbf{Parameter} & \textbf{Value} \\ \midrule
        Save Strategy                 & steps           \\
        Save Steps                    & 1000            \\
        Eval Strategy                 & steps           \\
        Learning Rate                 & 3e-5            \\
        Train Batch Size              & 2               \\
        Eval Batch Size               & 2               \\
        Epochs                        & 5               \\
        Weight Decay                  & 0.01            \\
        Eval Steps                    & 1000            \\
        Gradient Accumulation Steps   & 4               \\
        FP16                          & True            \\
        \bottomrule
    \end{tabular}
    \caption{Training Parameters}
    \label{tab:training_parameters}
\end{table}

